Number and location of pre-images under harmonic mappings in the plane

We derive a formula for the number of pre-images under a non-degenerate harmonic mapping $f$, using the argument principle. This formula reveals a connection between the pre-images and the caustics. Our results allow to deduce the number of pre-images under $f$ geometrically for every non-caustic point. We approximately locate the pre-images of points near the caustics. Moreover, we apply our results to prove that for every $k = n, n+1, \ldots, n^2$ there exists a harmonic polynomial of degree $n$ with $k$ zeros.

==> sect_argument_principle.tex <==
\subsection{The argument principle for harmonic mappings}

As usual, a curve is a continuous function $\gamma : \cc{a, b} \to \C$.
Let $f$ be a continuous and non-zero function on $\tr(\gamma)$, then the 
\emph{winding of $f$ on $\gamma$} is defined as the change of argument of 
$f(z)$ as $z$ travels along $\gamma$ from $\gamma(a)$ to $\gamma(b)$, divided 
by $2\pi$, i.e.,
\begin{equation} \label{eqn:winding}
W(f; \gamma) = \frac{1}{2 \pi} \Delta_\gamma \arg(f(z)) = \frac{1}{2 \pi} 
(\theta(b) - \theta(a)),
\end{equation}
where $\theta : \cc{a, b} \to \R$ is continuous with $\theta(t) = 
\arg(f(\gamma(t))$;
see~\cite[Sect.~2.3]{Balk1991} or~\cite[Ch.~7]{Beardon1979} for details.
The winding is also called the degree or topological degree of $f$ on $\gamma$; 
see~\cite[p.~3]{Lloyd1978} or~\cite[p.~29]{Sheil-Small2002}.

Denote the \emph{winding number} of a closed curve $\gamma$ about $\eta \in 
\C \setminus \tr(\gamma)$ by $\wn{\gamma}{\eta}$.
The winding number and the winding are related through
\begin{equation}\label{eqn:winding_winding_number}
W(f;\gamma) = \wn{f\circ\gamma}{0} \quad \text{and} \quad
\wn{\gamma}{\eta} = W(z \mapsto z-\eta; \gamma).
\end{equation}
In particular, $W(f; \gamma)$ is an integer if $\gamma$ is closed.

The argument principle for a continuous function $f$ 
relates the winding of $f$ to the indices of its exceptional points.
A point $z_0 \in \C$ is called an \emph{isolated exceptional point} of a 
function $f$, if $f$ is continuous and non-zero in some punctured neighborhood 
$D = \{ z \in \C : 0 < \abs{z - z_0} < r \}$ of $z_0$, and if
$f$ is either zero, not continuous, or not defined at $z_0$.
Then the \emph{Poincar\'e index} of $f$ at $z_0$ is defined as 
\begin{equation}
\ind(f;z_0) = W(f;\gamma),
\end{equation}
where $\gamma$ is a closed Jordan curve in $D$ about $z_0$ oriented in the 
positive sense, i.e., with $\wn{\gamma}{z_0} = 1$.
The Poincar\'e index is also called the index~\cite[Def.~2.2.2]{Lloyd1978} or 
the multiplicity~\cite[p.~44]{Sheil-Small2002}.
Similarly, $\infty$ is an isolated exceptional point of $f$, if $f$ is 
continuous and non-zero in $D = \{ z \in \C : \abs{z} > R \}$.  We define 
$\ind(f; \infty) = W(f; \gamma)$, where $\gamma$ is a 
closed Jordan curve in $D$ which is negatively oriented and surrounding the 
origin, such that $\infty$ lies on the left of $\gamma$ on the Riemann sphere;
see Figure~\ref{fig:poincare_infty}.
In either case the Poincar\'e index is independent of the choice of $\gamma$.
We get with $\varphi(z) = z^{-1}$
\begin{equation}\label{eqn:index_infty_phi}
\ind(f; \infty) = W(f; \gamma) = W(f \circ \varphi^{-1}; \varphi \circ \gamma)
= \ind(f \circ \varphi; 0).
\end{equation}
The Poincar\'e index generalizes the notion of the multiplicity of zeros 
and order of poles 
of an analytic function; see e.g.~\cite[p.~44]{Sheil-Small2002}.

\begin{figure}
\center
\input{fig_poincare_infty}
\caption{Poincar\'e index at $\infty$ visualized on the Riemann sphere 
$\widehat{\C}$.}\label{fig:poincare_infty}
\end{figure}


\begin{theorem}
Let $f$ be defined, continuous and non-zero on $\widehat{\C} = \C \cup \{ 
\infty \}$,
except for finitely many isolated exceptional points $z_1, \ldots, z_n$ in
$\widehat{\C}$, then
\begin{equation*}
\sum_{j=1}^n \ind(f; z_j) = 0.
\end{equation*}
\end{theorem}

This is similar to the fact that the sum of residues is zero for 
functions analytic in $\C$ except for finitely many isolated singularities; 
see~\cite[p.~53]{Markushevich1965}.



The following version of the argument principle for continuous functions can be 
obtained from~\cite[Sect.~2.3]{Balk1991}, or~\cite[Sect.~2.3]{Sheil-Small2002}. 
Special versions for harmonic mappings are given 
in~\cite{DurenHengartnerLaugesen1996} 
and~\cite[Thm.~2.2]{SuffridgeThompson2000}.

\begin{theorem}[Argument principle] \label{thm:winding}
Let $D$ be a multiply connected domain in $\widehat{\C}$ whose boundary 
consists of Jordan 
curves $\gamma_1, \ldots, \gamma_n$, which are oriented such that $D$ is on the 
left.
Let $f$ be continuous and non-zero in $\overline{D}$, except for finitely many 
exceptional points $z_1,\dots,z_k \in D$.  We then have
\begin{equation*}
\sum_{j=1}^n W(f; \gamma_j) = \sum_{j=1}^k \ind(f; z_j).
\end{equation*}
\end{theorem}



The only exceptional points of a harmonic mapping $f$ are its zeros and 
points where $f$ is not defined.
We begin with a result on the index of zeros; 
see~\cite[p.~413]{DurenHengartnerLaugesen1996} 
or~\cite[p.~66]{SuffridgeThompson2000}.

\begin{proposition}\label{prop:poincare_index_zeros}
Let $f$ be a harmonic mapping with a zero $z_0$, such that the local 
decomposition~\eqref{eqn:local_decomp} is of the form
\begin{equation*}
f(z) = \sum_{k=n}^\infty a_k (z-z_0)^k + \conj{\sum_{k=n}^\infty b_k 
(z-z_0)^k}, \quad n \geq 1,
\end{equation*}
where $a_n$ or $b_n$ can be zero, then
\begin{equation} \label{eqn:index_zero_in_N}
\ind(f; z_0) = \begin{cases}
+n &\text{ if } \abs{a_n} > \abs{b_n}, \\
-n &\text{ if } \abs{a_n} < \abs{b_n},
\end{cases}
\end{equation}
and, in particular,
\begin{equation} \label{eqn:index_nonsingular_zero}
\ind(f; z_0) = \begin{cases}
+1 &\text{ if $f$ is sense-preserving at } z_0, \\
-1 &\text{ if $f$ is sense-reversing at } z_0.
\end{cases}
\end{equation}
\end{proposition}

A zero $z_0$ of a harmonic 
mapping $f$ with $\ind(f; z_0) \in \Z\setminus\{-1,1\}$ is a singular zero by 
the above result.
Proposition~\ref{prop:poincare_index_zeros} covers non-singular zeros and the 
zeros in $\cM$; see~\eqref{eqn:omega_neq_1}.
If $\abs{a_n} = \abs{b_n} \neq 0$, then $z_0$ is a singular 
zero in $\cC \setminus \cM$,
in which case, the determination of the index is more challenging;
see~\cite{LuceSete2017} for the special case $f(z) = h(z) - \conj{z}$.

\begin{remark} \label{rem:zeros_in_M}
The zeros in $\cM$ can be interpreted as multiple zeros of $f$.
For a zero $z_0 \in \cM$ of $f$, there 
exists $r > 0$ such that $f$ is defined, non-zero and either sense-preserving 
or sense-reversing in $D = \{ z \in \C : 0 < \abs{z-z_0} \leq r \}$.
For $0 < \abs{\eps} < m = \min_{\abs{z-z_0} = r} \abs{f(z)}$ and $z$ with
$\abs{z - z_0} = r$ we have
\begin{equation*}
\abs{f(z) + \eps - f(z)} = \abs{\eps} < m \leq \abs{f(z)},
\end{equation*}
which implies $W(f + \eps; \gamma) = W(f; \gamma) = \ind(f; z_0)$ by Rouch\'e's 
theorem; see e.g.~\cite[Thm.~2.3]{SeteLuceLiesen2015a}.
Since $f + \eps$ has no poles in $\overline{D}$ and $f(z_0) + \eps \neq 0$, it 
has $\abs{\ind(f; z_0)}$ many distinct zeros in $D$ by the 
argument principle.
\end{remark}


Isolated exceptional points where $f$ is not defined are classified according 
to the limit $\lim_{z \to z_0} f(z)$; 
see~\cite[Def.~2.1]{SuffridgeThompson2000}, \cite[p.~44]{Sheil-Small2002}, and 
the classical notions for real-valued harmonic functions, e.g.~\cite[\S 
15.3, III]{Henrici1986}.

\begin{definition}\label{def:pole}
Let $f$ be a harmonic mapping in a punctured disk around $z_0 \in \C$.
Then $z_0$ is called
\begin{enumerate}
\item a \emph{removable singularity} of $f$, if $\lim_{z \to z_0} f(z) = c \in 
\C$,
\item a \emph{pole} of $f$, if $\lim_{z \to z_0} f(z) = \infty$,
\item an \emph{essential singularity} of $f$, if $\lim_{z \to z_0} f(z)$ does 
not exist.
\end{enumerate}
\end{definition}

If one defines $f(z_0) = c$ at a removable singularity, then $f$ is harmonic 
in~$z_0$; apply~\cite[Thm.~15.3d]{Henrici1986} to the real and imaginary parts 
of $f$.  In the sequel, we assume that removable singularities have been 
removed.
If $c = 0$, then $z_0$ is a zero of $f$, and still an exceptional point.

For most poles of harmonic mappings, the Poincar\'e index can be 
determined from the decomposition~\eqref{eqn:local_decomp_sing}.

\begin{proposition}\label{prop:poincare_index_poles}
Let $f$ be a harmonic mapping in a punctured neighborhood of $z_0$, such that
the local decomposition~\eqref{eqn:local_decomp_sing} is of the form
\begin{equation*}
f(z) = \sum_{\mathclap{k=-n}}^\infty a_k (z-z_0)^k
+ \conj{\sum_{\mathclap{k=-n}}^\infty b_k (z-z_0)^k} + c \log\abs{z-z_0},
\end{equation*}
where $a_{-n}$ or $b_{-n}$ can be zero, then
\begin{equation*}
\ind(f; z_0) = \begin{cases}
-n & \text{ if } n \geq 1 \text{ and } \abs{a_{-n}} > \abs{b_{-n}}, \\
+n & \text{ if } n \geq 1 \text{ and } \abs{a_{-n}} < \abs{b_{-n}}, \\
\phantom{+}0 & \text{ if } n = 0 \text{ and } c \neq 0.
\end{cases}
\end{equation*}
Moreover, in each case $z_0$ is a pole of $f$.
In the first case, $f$ is sense-preserving near $z_0$, and in the second it is 
sense-reversing near $z_0$.
In the third case, $z_0$ is an accumulation point of the critical set of $f$.
\end{proposition}

\begin{proof}
See~\cite[Lem.~2.2, 2.3, 2.4]{SuffridgeThompson2000} for the first two cases.
In the third case, we have $\ind(f; z_0) = 0$ if $n = 0$ and $c \neq 0$
by~\cite[pp.~70--71]{SuffridgeThompson2000}.
Moreover, $\omega$ can be continued analytically to $z_0 \notin \Omega$ with
$\abs{\omega(z_0)} = \lim_{z \to z_0} \abs{\omega(z)} = 1$, and hence $z_0$ 
is an accumulation point of the critical set of $f$.
\end{proof}

\begin{remark} \label{rem:singularities_on_crit}
If $n \geq 1$ and $\abs{a_{-n}} = \abs{b_{-n}} \neq 0$, we have that:
\begin{enumerate}
\item $z_0$ is an accumulation point of the critical set of $f$, as in the 
proof,

\item $z_0$ is a pole or an essential singularity of $f$, and both cases occur.
Consider $f_1(z) = z^2 + z^{-1} + \conj{z}^{-2}$ and
$f_2(z) = z^2 + z + \conj{z}^{-2}$, for which $z_0 = 0$ is an isolated 
exceptional point.
Since $\lim_{z \to 0} f_1(z) = \infty$, the origin is a pole of $f_1$ with 
$\ind(f_1; 0) = 0$; see~\cite[Ex.~2.6]{SuffridgeThompson2000}.
In contrast, $\lim_{z \to 0} f_2(z)$ does not exist (compare the limits on the 
real axis and the lines with $\re(z^{-2}) = 0$), i.e., $f_2$ has an essential 
singularity at $0$.
\end{enumerate}
\end{remark}

